DOMAINEVAL: An Auto-Constructed Benchmark for Multi-Domain Code Generation

Code benchmarks such as HumanEval are widely adopted to evaluate the capabilities of Large Language Models (LLMs), providing insights into their strengths and weaknesses. However, current benchmarks primarily exercise LLMs' capability on common coding tasks (e.g., bubble sort, greatest common divisor), leaving domain-specific coding tasks (e.g., computation, system, cryptography) unexplored. To fill this gap, we propose a multi-domain code benchmark, DOMAINEVAL, designed to evaluate LLMs' coding capabilities thoroughly. Our pipeline works in a fully automated manner, enabling a push-bottom construction from code repositories into formatted subjects under study. Interesting findings are observed by evaluating 12 representative LLMs against DOMAINEVAL. We notice that LLMs are generally good at computation tasks while falling short on cryptography and system coding tasks. The performance gap can be as much as 68.94% (80.94% - 12.0%) in some LLMs. We also observe that generating more samples can increase the overall performance of LLMs, while the domain bias may even increase. The contributions of this study include a code generation benchmark dataset DOMAINEVAL, encompassing six popular domains, a fully automated pipeline for constructing code benchmarks, and an identification of the limitations of LLMs in code generation tasks based on their performance on DOMAINEVAL, providing directions for future research improvements. The leaderboard is available at https://domaineval.github.io/.

==> sections/4_Related_Work.tex <==
\section{Related Work}

To assess the code generation capabilities of models, numerous code benchmarks were introduced such as APPS \citep{hendrycksMeasuringCodingChallenge2021} and CodeContests \citep{li2022competition}, which are datasets sourced from algorithmic design competitions that emphasize logical thinking. MBPP \citep{austinProgramSynthesisLarge2021} and HumanEval \citep{chenEvaluatingLargeLanguage2021} are datasets crafted manually for testing. These datasets are designed for evaluation, featuring highly independent functions and simplistic, idealized problem scenarios.
Standalone functions are predominantly focused on by these benchmarks; however, non-standalone functions are commonly encountered in pragmatic code generation scenarios \citep{yuCoderEvalBenchmarkPragmatic2024}.

Some other benchmarks attached importance on real-world problems by sourcing data from real scenarios such as StackOverflow, GitHub, and curating data manually to form benchmark datasets. For instance, PandasEval, NumpyEval \citep{zan2022cert}, and SecurityEval \citep{siddiq2022securityeval} are tailored benchmarks for specific scenarios \cite{zan2023large}. Focusing on specific scenarios is their limitation.

CoderEval \citep{yuCoderEvalBenchmarkPragmatic2024}, ClassEval \citep{du2023classeval}, DevEval \citep{li2024deveval}, and ODEX \citep{wang2023executionbased} were constructed in open domains, but they required significant investment of human labor in the stages of data curating, filtering, or annotation.

RepoEval \citep{zhangRepoCoderRepositoryLevelCode2023}, MultiPL-E \citep{multiPL}, and Exec-CSN \citep{xie2024codebenchgen} were constructed with little human involvement. However, RepoEval is focused on repository level task, which differs from ours. 
MultiPL-E obtained its data by translating other code datasets, and thus, it was not oriented towards open domains.
Exec-CSN employed LLMs to curate the CodeSearchNet dataset and generate test cases, resulting in a final dataset that has a gap from the real-world code on GitHub.

Moreover, previous benchmarks have not explored the difference of code generation capability of LLMs in multiple domains. Though a recent work~\cite{zhuoBigCodeBenchBenchmarkingCode2024} exercised capability of LLMs in using APIs from several domains, but its benchmark need human-LLM collaboration to construct. Our \name benchmark is designed not for tool utilization, but for concrete implementation of APIs and functions. Furthermore, \name can be constructed through a fully automated pipeline across open domains.

==> tables/result_pass_k_color.tex <==
\begin{table*}[h!]
\centering
\small
    \begin{tabular}{l|c|cccccc|cc}
    \toprule
    \textbf{Pass@1} (Greedy Search N=1) & \textbf{Size} & \textbf{Comp} & \textbf{Network} & \textbf{Visual} & \textbf{Basic} & \textbf{System} & \textbf{Crypt} & \textbf{Mean} & \textbf{Std} \\
    \midrule
    GPT-4o-mini & \textbackslash{} & \cellcolor[rgb]{ .569,  .667,  .875} 90.38  & \cellcolor[rgb]{ .682,  .753,  .91} 70.31  & \cellcolor[rgb]{ .741,  .8,  .925} 59.68  & \cellcolor[rgb]{ .686,  .761,  .91} 69.16  & \cellcolor[rgb]{ .788,  .835,  .941} 51.00  & \cellcolor[rgb]{ .831,  .871,  .953} 43.00  & \cellcolor[rgb]{ .957,  .702,  .51} 63.92  & \cellcolor[rgb]{ .949,  .976,  .929} 16.68  \\
    GPT-3.5-turbo & \textbackslash{} & \cellcolor[rgb]{ .608,  .698,  .886} 83.40  & \cellcolor[rgb]{ .745,  .804,  .925} 58.98  & \cellcolor[rgb]{ .8,  .843,  .941} 48.92  & \cellcolor[rgb]{ .761,  .816,  .933} 56.07  & \cellcolor[rgb]{ .89,  .918,  .969} 32.00  & \cellcolor[rgb]{ .898,  .922,  .973} 31.00  & \cellcolor[rgb]{ .98,  .863,  .769} 51.73  & \cellcolor[rgb]{ .859,  .933,  .804} 19.50  \\
    Qwen2-72B-Instruct-GPTQ-Int4 & 72B   & \cellcolor[rgb]{ .588,  .682,  .882} 86.86  & \cellcolor[rgb]{ .702,  .769,  .914} 66.80  & \cellcolor[rgb]{ .796,  .843,  .941} 49.46  & \cellcolor[rgb]{ .686,  .761,  .91} 69.16  & \cellcolor[rgb]{ .843,  .878,  .957} 41.00  & \cellcolor[rgb]{ .871,  .898,  .965} 36.00  & \cellcolor[rgb]{ .976,  .796,  .667} 58.21  & \cellcolor[rgb]{ .863,  .937,  .808} 19.39  \\
    DeepSeek-Coder-33b-instruct & 33B   & \cellcolor[rgb]{ .608,  .694,  .886} 83.93  & \cellcolor[rgb]{ .714,  .78,  .918} 64.45  & \cellcolor[rgb]{ .788,  .839,  .941} 50.54  & \cellcolor[rgb]{ .737,  .8,  .925} 59.81  & \cellcolor[rgb]{ .816,  .859,  .949} 46.00  & \cellcolor[rgb]{ .875,  .906,  .965} 35.00  & \cellcolor[rgb]{ .98,  .816,  .698} 56.62  & \cellcolor[rgb]{ .941,  .973,  .918} 16.94  \\
    DeepSeek-Coder-V2-Lite-Instruct & 16B   & \cellcolor[rgb]{ .596,  .686,  .882} 86.04  & \cellcolor[rgb]{ .725,  .788,  .922} 62.11  & \cellcolor[rgb]{ .792,  .839,  .941} 50.00  & \cellcolor[rgb]{ .71,  .776,  .918} 65.42  & \cellcolor[rgb]{ .843,  .878,  .957} 41.00  & \cellcolor[rgb]{ .859,  .89,  .961} 38.00  & \cellcolor[rgb]{ .98,  .812,  .69} 57.10  & \cellcolor[rgb]{ .91,  .957,  .875} 17.92  \\
    DeepSeek-Coder-6.7b-instruct & 6.7B  & \cellcolor[rgb]{ .608,  .698,  .886} 83.52  & \cellcolor[rgb]{ .745,  .804,  .925} 58.98  & \cellcolor[rgb]{ .816,  .859,  .949} 45.70  & \cellcolor[rgb]{ .749,  .808,  .929} 57.94  & \cellcolor[rgb]{ .871,  .898,  .965} 36.00  & \cellcolor[rgb]{ .847,  .882,  .957} 40.00  & \cellcolor[rgb]{ .984,  .851,  .757} 53.69  & \cellcolor[rgb]{ .929,  .969,  .902} 17.32  \\
    CodeLlama-34b-Instruct & 34B   & \cellcolor[rgb]{ .651,  .729,  .898} 76.07  & \cellcolor[rgb]{ .737,  .796,  .925} 60.16  & \cellcolor[rgb]{ .835,  .875,  .953} 41.94  & \cellcolor[rgb]{ .765,  .82,  .933} 55.14  & \cellcolor[rgb]{ .875,  .906,  .965} 35.00  & \cellcolor[rgb]{ .898,  .922,  .973} 31.00  & \cellcolor[rgb]{ .988,  .894,  .827} 49.89  & \cellcolor[rgb]{ .937,  .973,  .914} 17.09  \\
    CodeLlama-13b-Instruct & 13B   & \cellcolor[rgb]{ .627,  .71,  .894} 80.29  & \cellcolor[rgb]{ .725,  .788,  .922} 62.11  & \cellcolor[rgb]{ .835,  .871,  .953} 42.47  & \cellcolor[rgb]{ .745,  .804,  .925} 58.88  & \cellcolor[rgb]{ .882,  .91,  .969} 34.00  & \cellcolor[rgb]{ .918,  .937,  .976} 27.00  & \cellcolor[rgb]{ .988,  .886,  .812} 50.79  & \cellcolor[rgb]{ .847,  .929,  .784} 19.90  \\
    CodeLlama-7b-Instruct & 7B    & \cellcolor[rgb]{ .643,  .725,  .898} 77.13  & \cellcolor[rgb]{ .733,  .796,  .925} 60.55  & \cellcolor[rgb]{ .827,  .867,  .953} 43.55  & \cellcolor[rgb]{ .78,  .831,  .937} 52.34  & \cellcolor[rgb]{ .871,  .898,  .965} 36.00  & \cellcolor[rgb]{ .89,  .918,  .969} 32.00  & \cellcolor[rgb]{ .988,  .89,  .82} 50.26  & \cellcolor[rgb]{ .945,  .976,  .925} 16.82  \\
    CodeQwen1.5-7B-Chat & 7B    & \cellcolor[rgb]{ .6,  .69,  .886} 85.16  & \cellcolor[rgb]{ .733,  .792,  .925} 60.94  & \cellcolor[rgb]{ .804,  .851,  .945} 47.85  & \cellcolor[rgb]{ .733,  .796,  .925} 60.75  & \cellcolor[rgb]{ .863,  .894,  .961} 37.00  & \cellcolor[rgb]{ .863,  .894,  .961} 37.00  & \cellcolor[rgb]{ .984,  .839,  .733} 54.78  & \cellcolor[rgb]{ .898,  .953,  .855} 18.31  \\
    Phi-3-medium-4k-instruct & 14B   & \cellcolor[rgb]{ .651,  .733,  .902} 75.54  & \cellcolor[rgb]{ .737,  .796,  .925} 60.16  & \cellcolor[rgb]{ .82,  .863,  .949} 45.16  & \cellcolor[rgb]{ .729,  .792,  .922} 61.68  & \cellcolor[rgb]{ .835,  .875,  .953} 42.00  & \cellcolor[rgb]{ .875,  .906,  .965} 35.00  & \cellcolor[rgb]{ .984,  .855,  .765} 53.26  & 15.10  \\
    Llama-2-13b-chat & 13B   & \cellcolor[rgb]{ .624,  .71,  .89} 80.94  & \cellcolor[rgb]{ .776,  .827,  .937} 53.12  & \cellcolor[rgb]{ .875,  .906,  .965} 34.95  & \cellcolor[rgb]{ .82,  .863,  .949} 44.86  & \cellcolor[rgb]{ .965,  .973,  .992} 19.00  & 12.00  & 40.81  & \cellcolor[rgb]{ .678,  .847,  .553} 24.97  \\
    \midrule
    \textbf{Average} & \textbackslash{} & \cellcolor[rgb]{ .616,  .702,  .89} 82.44  & \cellcolor[rgb]{ .729,  .792,  .922} 61.56  & \cellcolor[rgb]{ .812,  .855,  .945} 46.69  & \cellcolor[rgb]{ .741,  .8,  .925} 59.27  & \cellcolor[rgb]{ .863,  .894,  .961} 37.50  & \cellcolor[rgb]{ .886,  .914,  .969} 33.08  & 53.42  & 18.33  \\
    \midrule
    \addlinespace
    \midrule
    \textbf{Pass@5} (Sampling Search N=5) & \textbf{Size} & \textbf{Comp} & \textbf{Network} & \textbf{Visual} & \textbf{Basic} & \textbf{System} & \textbf{Crypt} & \textbf{Mean} & \textbf{Std} \\
    \midrule
    GPT-4o-mini & \textbackslash{} & \cellcolor[rgb]{ .569,  .667,  .875} 91.26  & \cellcolor[rgb]{ .686,  .757,  .91} 72.66  & \cellcolor[rgb]{ .753,  .808,  .929} 61.83  & \cellcolor[rgb]{ .694,  .765,  .914} 71.03  & \cellcolor[rgb]{ .78,  .831,  .937} 57.00  & \cellcolor[rgb]{ .831,  .871,  .953} 49.00  & \cellcolor[rgb]{ .957,  .702,  .51} 67.13  & 14.75  \\
    GPT-3.5-turbo & \textbackslash{} & \cellcolor[rgb]{ .596,  .686,  .882} 87.33  & \cellcolor[rgb]{ .745,  .804,  .925} 62.89  & \cellcolor[rgb]{ .812,  .855,  .945} 52.15  & \cellcolor[rgb]{ .757,  .812,  .929} 60.75  & \cellcolor[rgb]{ .91,  .929,  .976} 36.00  & \cellcolor[rgb]{ .922,  .941,  .98} 34.00  & \cellcolor[rgb]{ .984,  .871,  .788} 55.52  & \cellcolor[rgb]{ .831,  .922,  .765} 19.74  \\
    Qwen2-72B-Instruct-GPTQ-Int4 & 72B   & \cellcolor[rgb]{ .576,  .675,  .878} 90.15  & \cellcolor[rgb]{ .698,  .765,  .914} 70.70  & \cellcolor[rgb]{ .796,  .843,  .941} 54.84  & \cellcolor[rgb]{ .678,  .753,  .906} 73.83  & \cellcolor[rgb]{ .824,  .863,  .949} 50.00  & \cellcolor[rgb]{ .847,  .882,  .957} 46.00  & \cellcolor[rgb]{ .965,  .745,  .58} 64.25  & \cellcolor[rgb]{ .929,  .969,  .898} 16.90  \\
    DeepSeek-Coder-33b-instruct & 33B   & \cellcolor[rgb]{ .58,  .675,  .878} 89.79  & \cellcolor[rgb]{ .698,  .765,  .914} 70.70  & \cellcolor[rgb]{ .792,  .839,  .941} 55.38  & \cellcolor[rgb]{ .714,  .776,  .918} 68.22  & \cellcolor[rgb]{ .78,  .831,  .937} 57.00  & \cellcolor[rgb]{ .875,  .902,  .965} 42.00  & \cellcolor[rgb]{ .965,  .753,  .588} 63.85  & \cellcolor[rgb]{ .949,  .976,  .925} 16.34  \\
    DeepSeek-Coder-V2-Lite-Instruct & 16B   & \cellcolor[rgb]{ .584,  .678,  .882} 88.91  & \cellcolor[rgb]{ .729,  .792,  .922} 65.62  & \cellcolor[rgb]{ .8,  .847,  .945} 53.76  & \cellcolor[rgb]{ .714,  .776,  .918} 68.22  & \cellcolor[rgb]{ .831,  .871,  .953} 49.00  & \cellcolor[rgb]{ .859,  .894,  .961} 44.00  & \cellcolor[rgb]{ .969,  .784,  .643} 61.59  & \cellcolor[rgb]{ .945,  .976,  .925} 16.35  \\
    DeepSeek-Coder-6.7b-instruct & 6.7B  & \cellcolor[rgb]{ .58,  .675,  .878} 89.79  & \cellcolor[rgb]{ .741,  .8,  .925} 63.67  & \cellcolor[rgb]{ .792,  .839,  .941} 55.38  & \cellcolor[rgb]{ .718,  .78,  .918} 67.29  & \cellcolor[rgb]{ .831,  .871,  .953} 49.00  & \cellcolor[rgb]{ .859,  .894,  .961} 44.00  & \cellcolor[rgb]{ .969,  .784,  .643} 61.52  & \cellcolor[rgb]{ .945,  .976,  .925} 16.36  \\
    CodeLlama-34b-Instruct & 34B   & \cellcolor[rgb]{ .608,  .698,  .886} 85.10  & \cellcolor[rgb]{ .741,  .8,  .925} 63.28  & \cellcolor[rgb]{ .835,  .871,  .953} 48.39  & \cellcolor[rgb]{ .745,  .804,  .929} 62.62  & \cellcolor[rgb]{ .878,  .906,  .965} 41.00  & \cellcolor[rgb]{ .875,  .902,  .965} 42.00  & \cellcolor[rgb]{ .98,  .851,  .749} 57.07  & \cellcolor[rgb]{ .929,  .969,  .902} 16.83  \\
    CodeLlama-13b-Instruct & 13B   & \cellcolor[rgb]{ .58,  .675,  .878} 89.85  & \cellcolor[rgb]{ .729,  .792,  .922} 65.62  & \cellcolor[rgb]{ .816,  .855,  .949} 51.61  & \cellcolor[rgb]{ .722,  .788,  .922} 66.36  & \cellcolor[rgb]{ .898,  .922,  .973} 38.00  & \cellcolor[rgb]{ .918,  .937,  .976} 35.00  & \cellcolor[rgb]{ .98,  .839,  .733} 57.74  & \cellcolor[rgb]{ .804,  .906,  .725} 20.55  \\
    CodeLlama-7b-Instruct & 7B    & \cellcolor[rgb]{ .596,  .69,  .886} 86.80  & \cellcolor[rgb]{ .741,  .8,  .925} 63.67  & \cellcolor[rgb]{ .816,  .855,  .949} 51.61  & \cellcolor[rgb]{ .733,  .796,  .925} 64.49  & \cellcolor[rgb]{ .867,  .898,  .961} 43.00  & \cellcolor[rgb]{ .886,  .914,  .969} 40.00  & \cellcolor[rgb]{ .976,  .831,  .722} 58.26  & \cellcolor[rgb]{ .914,  .961,  .882} 17.28  \\
    CodeQwen1.5-7B-Chat & 7B    & \cellcolor[rgb]{ .573,  .671,  .878} 91.03  & \cellcolor[rgb]{ .737,  .796,  .925} 64.06  & \cellcolor[rgb]{ .792,  .839,  .941} 55.38  & \cellcolor[rgb]{ .714,  .776,  .918} 68.22  & \cellcolor[rgb]{ .855,  .886,  .961} 45.00  & \cellcolor[rgb]{ .875,  .902,  .965} 42.00  & \cellcolor[rgb]{ .973,  .792,  .659} 60.95  & \cellcolor[rgb]{ .89,  .949,  .847} 17.95  \\
    Phi-3-medium-4k-instruct & 14B   & \cellcolor[rgb]{ .608,  .698,  .886} 85.10  & \cellcolor[rgb]{ .718,  .78,  .918} 67.58  & \cellcolor[rgb]{ .796,  .843,  .941} 54.30  & \cellcolor[rgb]{ .718,  .78,  .918} 67.29  & \cellcolor[rgb]{ .843,  .878,  .957} 47.00  & \cellcolor[rgb]{ .859,  .894,  .961} 44.00  & \cellcolor[rgb]{ .973,  .796,  .659} 60.88  & \cellcolor[rgb]{ .976,  .992,  .969} 15.45  \\
    Llama-2-13b-chat & 13B   & \cellcolor[rgb]{ .592,  .686,  .882} 87.68  & \cellcolor[rgb]{ .788,  .835,  .941} 55.86  & \cellcolor[rgb]{ .886,  .914,  .969} 39.78  & \cellcolor[rgb]{ .831,  .871,  .953} 48.60  & \cellcolor[rgb]{ .973,  .976,  .992} 26.00  & 21.00  & 46.49  & \cellcolor[rgb]{ .678,  .847,  .553} 24.10  \\
    \midrule
    \textbf{Average} & \textbackslash{} & \cellcolor[rgb]{ .588,  .682,  .882} 88.57  & \cellcolor[rgb]{ .729,  .792,  .922} 65.53  & \cellcolor[rgb]{ .808,  .851,  .945} 52.87  & \cellcolor[rgb]{ .729,  .792,  .922} 65.58  & \cellcolor[rgb]{ .855,  .89,  .961} 44.83  & \cellcolor[rgb]{ .882,  .91,  .969} 40.25  & 59.60  & 17.72  \\
    \bottomrule
    \end{tabular}%
\caption{\textbf{Pass@1} and \textbf{Pass@5} of LLMs against \name. We use \textit{Comp} for \textit{computation}, \textit{Visual} for \textit{visualization}, and \textit{Crypt} for \textit{cryptography}. \textbf{Mean} represents the macro-average of Pass@k across different domains, which is used to reflect the overall performance of LLMs. \textbf{Std} indicates the standard deviation of Pass@k across different domains, which is used to reflect the difference degree in performance of LLM across various domains. To highlight the differences, we use color scales.}
\label{tab:result_pass@k}
\end{table*}
